F{\AE}RDXEL: An Expert System for Danish Traffic Law

We present F{\AE}RDXEL, a tool for symbolic reasoning in the domain of Danish traffic law. F{\AE}RDXEL combines techniques from logic programming with a novel interface that allows users to navigate through its reasoning process, thereby ensuring the system's explainability. Towards the goal of better understanding the value of F{\AE}RDXEL, two evaluations of the system have been performed: (1) An empirical evaluation showing that for a selection of court cases, the conclusions of F{\AE}RDXEL align with those of Danish judges. (2) A qualitative evaluation from legal experts indicating that this work has potential to become a foundation for real-world AI tools supporting professionals in the Danish legal sector.

==> eptcsdata.tex <==
\providecommand{\firstpage}{383}
\providecommand{\publicationstatus}{M. Gebser, D. Inclezan, F. Ricca, M. Carro \& M. Truszczynski:\\
41st International Conference on Logic Programming (ICLP 2025)\\
EPTCS 439, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.439.26}{10.4204/EPTCS.439.26}}
\pdfoutput=1

